ViDA-MAN: Visual Dialog with Digital Humans

We demonstrate ViDA-MAN, a digital-human agent for multi-modal interaction, which offers realtime audio-visual responses to instant speech inquiries. Compared to traditional text or voice-based system, ViDA-MAN offers human-like interactions (e.g, vivid voice, natural facial expression and body gestures). Given a speech request, the demonstration is able to response with high quality videos in sub-second latency. To deliver immersive user experience, ViDA-MAN seamlessly integrates multi-modal techniques including Acoustic Speech Recognition (ASR), multi-turn dialog, Text To Speech (TTS), talking heads video generation. Backed with large knowledge base, ViDA-MAN is able to chat with users on a number of topics including chit-chat, weather, device control, News recommendations, booking hotels, as well as answering questions via structured knowledge.

==> conclusion.tex <==
\section{conclusion}
In this paper, we present a multi-modal interaction system powered by digital humans. The system receives user speech as input and intelligently responses through a multi-type spoken dialog system. Realistic human voice is generated by the TTS and high-fidelity appearance videos are rendered by our GAN-based system. The streaming system integrates everything and converts to media stream. We hope this demo can serve as a foundation for further study on multi-modal interaction.
